Scalable Microservice Forensics and Stability Assessment Using Variational Autoencoders

We present a deep learning based approach to containerized application runtime stability analysis, and an intelligent publishing algorithm that can dynamically adjust the depth of process-level forensics published to a backend incident analysis repository. The approach applies variational autoencoders (VAEs) to learn the stable runtime patterns of container images, and then instantiates these container-specific VAEs to implement stability detection and adaptive forensics publishing. In performance comparisons using a 50-instance container workload, a VAE-optimized service versus a conventional eBPF-based forensic publisher demonstrates 2 orders of magnitude (OM) CPU performance improvement, a 3 OM reduction in network transport volume, and a 4 OM reduction in Elasticsearch storage costs. We evaluate the VAE-based stability detection technique against two attacks, CPUMiner and HTTP-flood attack, finding that it is effective in isolating both anomalies. We believe this technique provides a novel approach to integrating fine-grained process monitoring and digital-forensic services into large container ecosystems that today simply cannot be monitored by conventional techniques

==> 4_implementation.tex <==
\section{Container Monitoring Framework}\label{implementation}

This is the implementation: spans pgs 2 to 3 (1 or 2 figures) 

 

==> futurework.tex <==
\section{Future Work}\label{futurework}
\noindent VAE latent models distill the most important feature information from each data sample. These latent models can be used as inputs to another classification model to perform any number of downstream tasks. In our case, we can put the container under artificial duress and record the resulting latent models. Treating the 'mode of duress' as a class label and the recorded latent model as the data sample, in theory we can do root cause analysis on the summarizer messages. This, along with designing a more robust VAE for 
